3DGSR: Implicit Surface Reconstruction with 3D Gaussian Splatting

In this paper, we present an implicit surface reconstruction method with 3D Gaussian Splatting (3DGS), namely 3DGSR, that allows for accurate 3D reconstruction with intricate details while inheriting the high efficiency and rendering quality of 3DGS. The key insight is incorporating an implicit signed distance field (SDF) within 3D Gaussians to enable them to be aligned and jointly optimized. First, we introduce a differentiable SDF-to-opacity transformation function that converts SDF values into corresponding Gaussians' opacities. This function connects the SDF and 3D Gaussians, allowing for unified optimization and enforcing surface constraints on the 3D Gaussians. During learning, optimizing the 3D Gaussians provides supervisory signals for SDF learning, enabling the reconstruction of intricate details. However, this only provides sparse supervisory signals to the SDF at locations occupied by Gaussians, which is insufficient for learning a continuous SDF. Then, to address this limitation, we incorporate volumetric rendering and align the rendered geometric attributes (depth, normal) with those derived from 3D Gaussians. This consistency regularization introduces supervisory signals to locations not covered by discrete 3D Gaussians, effectively eliminating redundant surfaces outside the Gaussian sampling range. Our extensive experimental results demonstrate that our 3DGSR method enables high-quality 3D surface reconstruction while preserving the efficiency and rendering quality of 3DGS. Besides, our method competes favorably with leading surface reconstruction techniques while offering a more efficient learning process and much better rendering qualities. The code will be available at https://github.com/CVMI-Lab/3DGSR.

==> main/exp_bak.tex <==
\section{Experiments}
\subsection{Experimental Settings}
\paragraph{Datasets}
Our evaluation encompasses three datasets: the NeRF synthetic dataset~\cite{mildenhall2021nerf}, the DTU real-captured dataset~\cite{jensen2014large}, and the Tanks\&Temples (TNT) large-scale dataset~\cite{knapitsch2017tanks}. The NeRF synthetic dataset consists of eight objects, each rendered via path tracing to generate 100 views. For testing, we select an eighth of these images, allocating the remainder for training. The DTU and TNT datasets are processed for camera poses as per~\cite{gao2023relightable}, with image and mask processing following the methodology outlined in~\cite{liu2020neural}. The image resolutions for the DTU and TNT datasets are $1600 \times 1200$ and $1920 \times 1080$ pixels, respectively.

\paragraph{Comparisons}
We evaluated our method from both surface reconstruction quality and rendering quality of novel-view synthesis.
We benchmark our algorithm against several state-of-the-art methods, including NeRF~\cite{mildenhall2021nerf}, NeuS~\cite{wang2021neus}, NeuSG~\cite{chen2023neusg}, RelighableGaussian~\cite{gao2023relightable}, and NeRF2Mesh~\cite{tang2022nerf2mesh}, Neuralangelo~\cite{li2023neuralangelo}, PET-NeuS~\cite{wang2023petneus}, BakedSDF~\cite{yariv2023bakedsdf}, VolSDF~\cite{yariv2021volume}. 
% We evaluate different approaches regarding their novel-view synthesis and surface reconstruction qualities. 
The quality of image synthesis is quantified using the Peak Signal-to-Noise Ratio (PSNR). For surface reconstruction accuracy, we employ the Chamfer distance and the F1 score as our metrics~\cite{knapitsch2017tanks}. Furthermore, we also compare the rendering quality of our method with some works that solely focus on novel view synthesis tasks (Tri-MipRF~\cite{hu2023tri}, Zip-NeRF~\cite{barron2023zipnerf}, 3DGS~\cite{kerbl3Dgaussians}).


\begin{table*}[h]
  \centering
  \begin{tabular}{l|lccccccccc}
    \toprule[1pt]
                    & & Chair & Drums & Ficus & Hotdog & Lego & Materials & Mic & Ship & Avg\\
    \hline
    \multirow{9}{*}{\rotatebox[origin=c]{90}{PSNR}}  
    &NeRF~\cite{mildenhall2021nerf}              & 34.17 & 25.08 & 30.39 & 36.82 & 33.31 & \cellcolor{yzysecond}30.03 & 34.78 & 29.30 & 31.74 \\
    &Ins-NGP~\cite{muller2022instant}           & \cellcolor{yzythird}35.00 & \cellcolor{yzysecond}26.02 & \cellcolor{yzysecond}33.51  & \cellcolor{yzythird}37.40 & \cellcolor{yzybest}36.39 &29.78 &\cellcolor{yzysecond}36.22 &\cellcolor{yzybest}31.10 &\cellcolor{yzysecond}33.18 \\
    &Mip-NeRF~\cite{barron2021mip}          & \cellcolor{yzysecond}35.14 & \cellcolor{yzythird}25.48 & \cellcolor{yzythird}33.29 & \cellcolor{yzysecond}37.48 & \cellcolor{yzythird}35.70 & \cellcolor{yzybest}30.71 & \cellcolor{yzybest}36.51 & \cellcolor{yzythird}30.41 & \cellcolor{yzythird}33.09 \\
    &3D-GS~\cite{kerbl3Dgaussians}          & \cellcolor{yzybest}35.36 & \cellcolor{yzybest}26.15 & \cellcolor{yzybest}34.87 & \cellcolor{yzybest}37.72 & \cellcolor{yzysecond}35.78 & \cellcolor{yzythird}30.00 & \cellcolor{yzythird}35.36 & \cellcolor{yzysecond}30.80 & \cellcolor{yzybest}33.32 \\\hhline{~|*9{-}-|}
    &NeuS~\cite{wang2021neus}              & \cellcolor{yzythird}31.22 & \cellcolor{yzythird}24.85 & \cellcolor{yzythird}27.38  & \cellcolor{yzysecond}36.04    & \cellcolor{yzythird}34.06 & \cellcolor{yzysecond}29.59 & \cellcolor{yzythird}31.56 & \cellcolor{yzythird}26.94 & \cellcolor{yzythird}30.20 \\
    &NeRO~\cite{wang2021neus}              & \cellcolor{yzythird}31.22 & \cellcolor{yzythird}24.85 & \cellcolor{yzythird}27.38  & \cellcolor{yzysecond}36.04    & \cellcolor{yzythird}34.06 & \cellcolor{yzysecond}29.59 & \cellcolor{yzythird}31.56 & \cellcolor{yzythird}26.94 & \cellcolor{yzythird}30.20 \\
    &VolSDF~\cite{wang2021neus}              & \cellcolor{yzythird}31.22 & \cellcolor{yzythird}24.85 & \cellcolor{yzythird}27.38  & \cellcolor{yzysecond}36.04    & \cellcolor{yzythird}34.06 & \cellcolor{yzysecond}29.59 & \cellcolor{yzythird}31.56 & \cellcolor{yzythird}26.94 & \cellcolor{yzythird}30.20 \\
    &BakedSDF~\cite{wang2021neus}              & \cellcolor{yzythird}31.22 & \cellcolor{yzythird}24.85 & \cellcolor{yzythird}27.38  & \cellcolor{yzysecond}36.04    & \cellcolor{yzythird}34.06 & \cellcolor{yzysecond}29.59 & \cellcolor{yzythird}31.56 & \cellcolor{yzythird}26.94 & \cellcolor{yzythird}30.20 \\
    &NeRF2Mesh~\cite{tang2022nerf2mesh}         & \cellcolor{yzysecond}34.25 & \cellcolor{yzysecond}25.04 & \cellcolor{yzysecond}30.08  & \cellcolor{yzythird}35.70    & \cellcolor{yzybest}34.90 & \cellcolor{yzythird}26.26 & \cellcolor{yzysecond}32.63 & \cellcolor{yzysecond}29.47 & \cellcolor{yzysecond}30.88\\
    % &Ours              & 34.07 & 25.93 & 34.92 & 36.40 & 34.61 & 29.54 & 35.97 & 30.94 & 32.79 \\
    &Ours & \cellcolor{yzybest}34.85 & \cellcolor{yzybest}26.08 & \cellcolor{yzybest}35.17 & \cellcolor{yzybest}36.88 & \cellcolor{yzybest}34.90 & \cellcolor{yzybest}30.03 & \cellcolor{yzybest}36.44 & \cellcolor{yzybest}31.48 & \cellcolor{yzybest}33.23 \\
    \bottomrule[1pt]
    \multirow{5}{*}{\rotatebox[origin=c]{90}{C-$\mathcal{L}_1$}} 
    &NeRO~\cite{wang2021neus}              & \cellcolor{yzythird}31.22 & \cellcolor{yzythird}24.85 & \cellcolor{yzythird}27.38  & \cellcolor{yzysecond}36.04    & \cellcolor{yzythird}34.06 & \cellcolor{yzysecond}29.59 & \cellcolor{yzythird}31.56 & \cellcolor{yzythird}26.94 & \cellcolor{yzythird}30.20 \\
    &VolSDF~\cite{wang2021neus}              & \cellcolor{yzythird}31.22 & \cellcolor{yzythird}24.85 & \cellcolor{yzythird}27.38  & \cellcolor{yzysecond}36.04    & \cellcolor{yzythird}34.06 & \cellcolor{yzysecond}29.59 & \cellcolor{yzythird}31.56 & \cellcolor{yzythird}26.94 & \cellcolor{yzythird}30.20 \\   
    &NeuS~\cite{wang2021neus} & 3.99 & \cellcolor{yzythird}1.27 & \cellcolor{yzythird}0.94 & \cellcolor{yzysecond}2.12 & 2.56 & \cellcolor{yzysecond}1.39 & \cellcolor{yzysecond}1.00 & 5.38 & 2.33 \\
    &BakedSDF~\cite{wang2021neus}              & \cellcolor{yzythird}31.22 & \cellcolor{yzythird}24.85 & \cellcolor{yzythird}27.38  & \cellcolor{yzysecond}36.04    & \cellcolor{yzythird}34.06 & \cellcolor{yzysecond}29.59 & \cellcolor{yzythird}31.56 & \cellcolor{yzythird}26.94 & \cellcolor{yzythird}30.20 \\
    &NeRF2Mesh~\cite{tang2022nerf2mesh} & \cellcolor{yzysecond}1.62 & \cellcolor{yzysecond}1.11 & \cellcolor{yzybest}0.65 & \cellcolor{yzythird}2.73 & \cellcolor{yzythird}1.93 & \cellcolor{yzythird}1.42 & \cellcolor{yzybest}0.78 & \cellcolor{yzybest}2.20 & \cellcolor{yzysecond}1.55 \\
    &RelightableGaussian~\cite{gao2023relightable} & \cellcolor{yzythird}3.65 & 2.34 & 1.26 & 3.11 & \cellcolor{yzysecond}1.63 & \cellcolor{yzybest}1.35 & 1.76 & \cellcolor{yzysecond}3.35 & \cellcolor{yzythird}2.31\\
    &Ours & \cellcolor{yzybest}1.01 & \cellcolor{yzybest}0.95 & \cellcolor{yzysecond}0.69 & \cellcolor{yzybest}1.95 & \cellcolor{yzybest}1.54 & \cellcolor{yzythird}1.42 & \cellcolor{yzythird}1.15 & \cellcolor{yzythird}3.53 & \cellcolor{yzybest}1.53 \\
    \bottomrule[1pt]
 %\bottomrule[1pt]
  \end{tabular}
  \vspace{+0.3cm}
  \caption{We assess the quality of synthesized images and the accuracy of surface reconstruction, with each cell colored to indicate the \colorbox{yzybest}{best}, \colorbox{yzysecond}{second best}, and \colorbox{yzythird}{third best}. Our method is compared against various state-of-the-art (SOTA) approaches in tasks of novel view synthesis and surface reconstruction. It outperforms all competitors in both tasks, achieving the highest PSNR and the lowest Chamfer-$\mathcal{L}_1$ (C-$\mathcal{L}_1$) distance.}
  \label{tab: all in NeRF Synthetic}
\end{table*}

\begin{table*}[h]
\centering
\begin{tabular}{@{}lcccccccccccccccc@{}}
\toprule
{Scan ID}     & {24} & {37} & {40} & {55} & {63} & {65} & {69} & {83} & {97} & {105} & {106} & {110} & {114} & {118} & {122} & {Mean} \\ \hline
COLMAP            & \cellcolor{yzysecond}0.81        & 2.05        & \cellcolor{yzysecond}0.73        & 1.22        & 1.79        & 1.58        & 1.02 & 3.05        & 1.40        & 2.05        & 1.00         & 1.32         & 0.49         & 0.78         & 1.17         & 1.36          \\
 NeRF~\cite{mildenhall2021nerf} & 1.90 & {1.60} & {1.85} & {0.58} & {2.28} & {1.27} & {1.47} & {1.67} & {2.05} & {1.07} & {0.88} & {2.53} & {1.06} & {1.15} & {0.96} & {1.49} \\
NeuS \cite{wang2021neus}    & \cellcolor{yzythird}1.00        & \cellcolor{yzythird}1.37        & 0.93        & \cellcolor{yzysecond}0.43        & \cellcolor{yzybest}1.10        & \cellcolor{yzybest}0.65        & \cellcolor{yzybest}0.57 & \cellcolor{yzysecond}1.48        & \cellcolor{yzybest}1.09        & \cellcolor{yzysecond}0.83         & \cellcolor{yzybest}0.52         & \cellcolor{yzythird}1.20         & \cellcolor{yzybest}0.35         & \cellcolor{yzybest}0.49         & \cellcolor{yzybest}0.54         & \cellcolor{yzysecond}0.84          \\
VolSDF \cite{yariv2021volume}  & 1.14        & \cellcolor{yzysecond}1.26        & \cellcolor{yzythird}0.81        & \cellcolor{yzythird}0.49        & \cellcolor{yzythird}1.25        & \cellcolor{yzysecond}0.70        & \cellcolor{yzysecond}0.72        & \cellcolor{yzybest}1.29        & \cellcolor{yzysecond}1.18        & \cellcolor{yzybest}0.70         & \cellcolor{yzysecond}0.66         & \cellcolor{yzysecond}1.08         & \cellcolor{yzysecond}0.42         & \cellcolor{yzysecond}0.61         & \cellcolor{yzysecond}0.55         & \cellcolor{yzythird}0.86          \\
ReGS \cite{gao2023relightable}  & 1.14        & \cellcolor{yzysecond}1.26        & \cellcolor{yzythird}0.81        & \cellcolor{yzythird}0.49        & \cellcolor{yzythird}1.25        & \cellcolor{yzysecond}0.70        & \cellcolor{yzysecond}0.72        & \cellcolor{yzybest}1.29        & \cellcolor{yzysecond}1.18        & \cellcolor{yzybest}0.70         & \cellcolor{yzysecond}0.66         & \cellcolor{yzysecond}1.08         & \cellcolor{yzysecond}0.42         & \cellcolor{yzysecond}0.61         & \cellcolor{yzysecond}0.55         & \cellcolor{yzythird}0.86          \\
% MonoSDF (MLP) & 0.83 & {1.61} & {0.65} & {0.47} & {0.92} & {0.87} & {0.87} & {1.30} & {1.25} & {0.68} & \textbf{0.65} & {0.96} & {0.41} & {0.62} & {0.58} & {0.84} \\
Ours & \cellcolor{yzybest}0.68 & \cellcolor{yzybest}0.84 & \cellcolor{yzybest}0.70 & \cellcolor{yzybest}0.39 & \cellcolor{yzysecond}1.16 & \cellcolor{yzythird}0.87 & \cellcolor{yzythird}0.77 & \cellcolor{yzysecond}1.48 & \cellcolor{yzythird}1.26 & \cellcolor{yzythird}0.87 & \cellcolor{yzythird}0.69 & \cellcolor{yzybest}0.80 & \cellcolor{yzysecond}0.42 & \cellcolor{yzythird}0.64 & \cellcolor{yzythird}0.60 & \cellcolor{yzybest}0.81 \\
\bottomrule
\end{tabular}
\caption{Quantitative assessment on the DTU dataset with each cell colored to indicate the \colorbox{yzybest}{best}, \colorbox{yzysecond}{second best}, and \colorbox{yzythird}{third best}. Our method achieves the highest average quality of surface reconstruction and the lowest Chamfer-$\mathcal{L}_1$ distance with real-world data.}
\label{tab: all in dtu}
\end{table*}

\begin{figure*}
	\centering
	% \vspace{-3mm}
	\includegraphics[width=1.\linewidth]{Figure/vs_nerf2mesh.pdf}
	% \vspace{-3mm}
	\caption{Qualitative comparisons of reconstructed results between NeRF2Mesh~\cite{tang2022nerf2mesh}, Relightable 3D Gaussian~\cite{gao2023relightable}, and our method on the NeRF Synthetic dataset. Our method yields the highest-quality surface reconstruction preserving fine details and intricate structures.}
\label{fig:recon_exp}
	% \vspace{-5mm}
\end{figure*}

\begin{figure*}
	\centering
	% \vspace{-3mm}
	\includegraphics[width=1.\linewidth]{Figure/DTU_Results.pdf}
	% \vspace{-3mm}
	\caption{Qualitative comparisons of reconstructed results between VolSDF~\cite{yariv2021volume}, Relightable 3D Gaussian~\cite{gao2023relightable}, and our method on the DTU dataset. Our method yields the highest-quality surface reconstruction preserving fine details and intricate structures.}
\label{fig: DTU}
	% \vspace{-5mm}
\end{figure*}

\paragraph{Implementation Details}
Our work is implemented by PyTorch and CUDA and optimized by AdamW optimizer. 
We bind the Gaussian points to the SDF field for the whole training process to ensure that the Gaussian rendering process can provide a coarse SDF field, that can boost the converging speed of volumetric rendering.
To ensure stable optimization, we introduce the warm-up strategy to make sure the dynamic Gaussian points can move around to the surface and provide an accurate supervised signal.
The warm-up steps are set as 3000 for the Nerf synthetic dataset and 5000 for the TNT dataset.
During the volumetric rendering stage, we sample $N=1024$ rays per step.


For the synthetic data, we initialize the implicit function as a sphere, and the position of Gaussian is determined by the zero-level surface of the SDF field.
For the real-world scenes, which frequently exhibit intricate geometry and noised pose, we adopt the SFM points as the initialized Gaussian position, and the network is still initialized as a sphere.
Furthermore, we also apply the sparse MVS points to ensure the consistency between the rendered depth $\mathcal{D}$ and projected depth map $D_{mvs}$ with $\mathcal{L}_1$ loss.
Our models are trained for 30000 iterations, and all the experiments are conducted on a single NVIDIA GeForce RTX 3090 GPU.

\subsection{Ablation Study}
We conduct ablation studies on the NeRF Synthetic dataset in Table~\ref{tab: ablation} to evaluate the effectiveness of each module in our method. Six different configurations are investigated to train our model. 

\paragraph{Volumetric Constraints.} The volumetric constraints have a minimal impact on novel view synthesis (PSNR: 32.83-33.32) yet significantly influence the reconstruction results (Chamfer-L1: 3.63-1.51). Both 3DGS rasterization and ray-based volumetric rendering rely on image supervision. However, the depth and normal representations derived from these dual methods exhibit distinct characteristics. While 3DGS excels at capturing high-frequency signals, it often suffers from floaters. Conversely, ray-based volumetric rendering yields smoother and more stable outcomes, but may struggle to capture fine details.

These two methods can complement each other and help address their respective weaknesses. Redundant Gaussian points can be effectively eliminated, and simultaneously, the high-frequency information learned by 3DGS can be employed to enhance the quality of the SDF field. This is demonstrated in Table 1 and Figure 3 of the main paper.

% We see that (1) reducing volumetric constraints will get great rendering results but worse reconstruction results. 
\paragraph{Learnable $\beta$.} {By making $\beta$ trainable results, the conversion from SDF to 3DGS opacity can be learned automatically, which results in a 0.20 and 0.44 improvement in rendering and reconstruction performance, respectively. }

\paragraph{Normal Supervision.} If we use the pseudo normal to supervise the normal of Gaussian points, the model will get 0.23 and 0.05 improvement in Chamfer-$\mathcal{L}_1$ and PSNR, respectively.

\paragraph{Eikonal Loss.} {Removing the eikonal loss (Eq.~\eqref{eq: eikonal}) will relax the constraint of SDF field, which can damage the surface learning and lead to worse reconstruction results. Note that better rendering quality (PSNR 33.4) is obtained in this configuration, which indicates the relaxation of geometric constraints in specific ways can aid in improving rendering quality.}

\paragraph{Surface Alignment.} Constraining the Gaussian points close to the zero-level surface will inject more high-frequency information into the SDF field leading to detailed surface extracted results. 

\paragraph{Reconstruction Strategy.} {Compared with the marching cube with the SDF field, we also employ Poisson reconstruction to extract the surface from Gaussians with normals derived from the implicit SDF field, which exhibits a lower performance.}
This can be attributed to the noisy, sparse distribution of Gaussians that significantly impact the surface reconstruction quality. 
In contrast, the implicit SDF field provides a continuous representation, allowing for easy extraction of high-fidelity surfaces.
\begin{table}[h]
    \centering 
    \begin{tabular}{lccccc}
        \bottomrule[0.9pt]
        Method & Chamfer-$\mathcal{L}_1$ & F-score & PSNR & LPIPS & SSIM \\ 
        \hline
        w/o Geo                      & 3.63 & 80.20   & 32.83 & 0.0380  & 0.963 \\
        % \hline
         static $\beta$              & 1.95 & 90.20   & 33.02 & 0.0385  & 0.966 \\
        % \hline
        w/o eq~\eqref{eq:normalloss} & 1.74 & 91.36  & 33.18 & 0.0383  & 0.967 \\
        % \hline
         w/o eq~\eqref{eq: eikonal}  & 2.00  & 87.89  & \textbf{33.40}  & 0.0350   & \textbf{0.968} \\
        % \hline
         w/o eq~\eqref{eq: point}    & 1.69 & 91.70   & 33.06 & 0.0388  & 0.966 \\
        % \hline
         Poisson                     & 2.03 & 87.86  & -     & -       & - \\
        % \hline
        \emph{Ours (full)}           & \textbf{1.51} & \textbf{93.50} &33.23& \textbf{0.034} & \textbf{0.968}\\
        \toprule[0.9pt]
    \end{tabular}
    \caption{Ablation study on the NeRF Synthetic dataset, where we evaluate the effect of each proposed component.}
    \label{tab: ablation}
\end{table}

\subsection{Experimental Results}
Tables~\ref{tab: all in NeRF Synthetic} and~\ref{tab: all in dtu} present the quantitative results for synthetic and real-world datasets, respectively. On synthetic data, Table~\ref{tab: all in NeRF Synthetic} demonstrates that our method surpasses other state-of-the-art methods in terms of the reconstruction quality, as measured by Chamfer-$\mathcal{L}_1$ distance. Furthermore, our method also excels in synthesizing high-quality novel view images, which are comparable to state-of-the-art novel view synthesis methods. This highlights our method's superiority over surface reconstruction techniques and its competitive performance in novel view synthesis tasks. 
On real-captured DTU datasets, as shown in Table~\ref{tab: all in dtu}, our method also exhibits the best performance in terms of average surface reconstruction quality. 


Additionally, we provide qualitative comparisons of the reconstruction results qualitatively and present them in Figure~\ref{fig:recon_exp}. 
The state-of-the-art NeRF-based 3D reconstruction method NeRF2Mesh~\cite{tang2022nerf2mesh} fails to preserve fine details like fine Mic textures, Lego tracks, and stripes on the Hotdog disk.
RelightableGaussian~\cite{gao2023relightable} incorporates shading equations to determine Gaussian appearance and trains 3D Gaussians with attributes of normal and BRDF. 3D surfaces can then be obtained by applying Screened Poisson Reconstruction~\cite{kazhdan2013screened} on the 3D Gaussians assigned with normal. However, Gaussians are naturally discontinuous and unstructured, resulting in broken parts on the Mic and floaters on the Hotdog disk. Due to the absence of smooth surface modeling, its reconstructed results on Lego tracks, which contain intricate structures, are noisy and inaccurate. Combining the fitting power of Gaussian Splatting and the smooth surface modeling of the implicit SDF field, our method reconstructs surfaces with geometric details accurately and smoothly.


% \begin{table}
%   \centering
%   \begin{tabular}{|c|c|c|}
%     \hline
%     \multirow{3}{*}{\rotatebox[origin=c]{90}{PSNR}} & Column 2 & Column 3 \\
%     & Data 1 & Data 2 \\
%     & Data 3 & Data 4 \\
%     \hline
%   \end{tabular}
%   \caption{Example table with vertical text in the first column.}
%   \label{tab:vertical_text}
% \end{table}
